Igusa integrals and volume asymptotics in analytic and adelic geometry

We establish asymptotic formulae for volumes of height balls in analytic varieties over local fields and in adelic points of algebraic varieties over number fields, relating the Mellin transforms of height functions to Igusa integrals and to global geometric invariants of the underlying variety. In the adelic setting, this involves the construction of general Tamagawa measures.

==> notations.tex <==
$X$, variety

$F$, local field, number field

$S$, finite set of places in a number field, usually including the archimedean ones

$\mathfrak o_F$, $\mathfrak o_{F,S}$, set of integers in $F$, of
$S$-integers

$v$, place

$F_v$, completion of a number field $F$ at a place~$v$

$\mathfrak o_v$, ring of integers in $F_v$

$k_v$, residue field at a place $v$

$q_v$, cardinality of $k_v$

$\AD_F$, $\AD_F^S$,  adeles of a number field $F$, adeles outside $S$

$\Gamma_F$, absolute Galois group of~$F$

$\EP (U)$, virtual Galois-module attached to a smooth variety $U$

$\Phi_v\in\Gamma_F$, Frobenius element at the place~$v$

$\mathrm L(s,\cdot)$, $\mathrm L^S(s,\cdot)$, $\mathrm L^{S,*}(1,\cdot)$,
Artin L-function, outside $S$, its leading term at $s=1$,

$\mu_v$, local measures on a smooth variety,
defined by a metric on the anticanonical line bundle

$\tau$, $\tau^S$, Tamagawa measure on the adelic points of a
smooth algebraic variety

--------

$\Aff^n$, $\Aff^n_F$, affine $n$-space, affine $n$-space over a field~$F$

$D_\alpha$, boundary divisors

$\mathscr A$, set of indices $\alpha$ indexing the boundary divisors

$F_\alpha$, splitting field of $D_\alpha$,

$\mathsec f_\alpha$, canonical section of $\mathscr O(D_\alpha)$,

$\mathbf s=(s_\alpha)$, coordinates of a complexified line bundle.

%$H(\mathbf x;\mathbf s)$, height of an adelic point with respect
%to a complexified line-bundle with coordinates $\mathbf s$

$\mathfrak u_v$, relevant local points in $U(F_v)$
($(Z,\mathfrak o_v)$-integral points if $v\not\in S$)

$\mathscr A_Z\subset\mathscr A$, such that $Z=\sum_{\alpha\in\mathscr A_Z}
D_\alpha$,

$\Tube(\Omega)$, if $\Omega$ is a subset of a $\R$-vector space $V$,
then $\Tube(\Omega)=\Omega+\mathrm i V$ in $V\otimes\C$



